Systematic and Statistical Uncertainties of the Hilbert-Transform Based High-precision FID Frequency Extraction Method

Pulsed nuclear magnetic resonance (NMR) is widely used in high-precision magnetic field measurements. The absolute value of the magnetic field is determined from the precession frequency of nuclear magnetic moments. The Hilbert transform is widely used to extract the phase function from the observed free induction decay (FID) signal and then its frequency. In this paper, a detailed implementation of a Hilbert-transform based FID frequency extraction method is described. How artifacts and noise level in the FID signal affect the extracted phase function are derived analytically. A method of mitigating the artifacts in the extracted phase function of an FID is discussed. Correlations between noises of the phase function samples are studied for different noise spectra. We discovered that the error covariance matrix for the extracted phase function is nearly singular and improper for constructing the $\chi^2$ used in the fitting routine. A down-sampling method for fixing the singular covariance matrix has been developed, so that the minimum $\chi^2$-fit yields properly the statistical uncertainty of the extracted frequency. Other practical methods of obtaining the statistical uncertainty are also discussed.

==> MethodBackup.tex <==
\section{FID Frequency Extraction Method}
\label{sec:method}

In a uniform magnetic field, the FID signal $f(t)$ can be modeled as
\begin{align}
f(t)=A\exp(-t/T_{2})\exp\left(i(\omega t+\phi_0)\right)\label{eq:fid_uniform}, 
\end{align}
where $\omega$ is the nuclear spin precession angular frequency after the down-mixing, and $A$ is its initial signal amplitude. The decay time constant $T_{2}$ describes the relaxation of the transverse component of the nuclear spin polarization \cite{Slichter:1990}, and it depends on the detection material. %If the FID signal is mixed-down before digitization, $\omega$ is the NMR frequency after the down mixing. 
%The oscillation factor $\exp(i(\omega t+\phi_0))$ of the FID is expressed in the complex form to simplify later derivations, and the physical signal $f_r$ is the real part of this complex function. 
The function $f(t)$ is complex, and the measured signal is its real part $f_r$. If the magnetic field is not uniform, signals generated by different parts of the detection material have different frequencies and amplitudes. Suppose the signal generated by spin precessions within an angular frequency range $(\omega,\omega+d\omega)$ has an amplitude of $g(\omega)d\omega$, the net signal is given by the superposition
\begin{align}
f(t)&=N\exp(-\frac{t}{T_{2}})\int_{-\infty}^{+\infty}g(\omega)\exp(i(\omega t + \phi_0))d\omega,\label{eq:fid_nonuniform}
\end{align}
where $N$ is a normalization constant. The FID function can be expressed in the form of a general complex function
\begin{align}
    f(t)=A(t)\exp(i\Phi(t)),
    \label{eq:general_complex}
\end{align}
where $A(t)$ and $\Phi(t)$ are real. According to Ref.~\cite{Cowan_1996}, the average NMR frequency $\bar{\omega}$ weighted by $g(\omega)$ can be determined by calculating the derivative of $\Phi(t)$ at $t=0$:
\begin{align}
    \bar{\omega}&=\int_{-\infty}^{+\infty}\omega g(\omega)d\omega\\
    &=\left. \frac{d\Phi(t)}{dt} \right| _{t=0},
\end{align}
and $t=0$ corresponds to the time when the $\pi/2$-pulse starts. This average frequency corresponds to the average field sensed by the probe weighted by the signal amplitude for the frequency interval. 

%Assume the magnetic field being measured is in the $hat{y}$-direction, and the axial of the NMR probe coil is along the $\hat{z}$-direction. The $\pi/2$-pulse flips the magnetic polarization due to the proton magnetic moment from the $\hat{y}$ direction into the $x-z$ plane. After the $\pi/2$-pulse, the FID signal generated by the precession of the nuclear magnetic polarization can be modeled as 
%\begin{align}
%f(t)&=A\exp(-\frac{t}{\tau})\exp(i(\Omega t + \phi_0)),\label{eq:fid_uniform}\\
%\frac{1}{\tau}&=\frac{1}{T_1}+\frac{1}{T_2},\nonumber
%\end{align}
%where $\Omega$ is the NMR frequency, and $\phi_0$ is a constant initial phase. If the FID is mixed with a standard-frequency signal, then $\Omega=\omega_{s}-\omega_{R}$. The time constants $T_1$ and $T_2$ depend on the detection material, but not the nonuniformity of the magnetic field. Eq.~\ref{eq:fid_uniform} uses the complex form to simplify the calculation, and the physical signal is the real part of it. 

%In a non-uniform field, protons at different positions precess at different angular frequencies. The amplitude contributions from different positions are also different, because the $\pi/2$-pulse strength, sensitivity of the coil, and potentially the detection material distribution are not uniform. For a macroscopically small volume $dV=dxdydz$ in which the magnetic field non-uniformity is negligible, the signal generated in this volume can still be modeled by Eq.~\ref{eq:fid_uniform}. At the macroscopic distance the magnetic field generated by the precessing nuclear magnetic polarization is rather small comparing to the main magnetic field, so the signals generated by different volumes are independent and the total signal is the superposition of them:
%\begin{align}
%    f(t)&=\exp(-\frac{t}{\tau})\iiint_{-\infty}^{+\infty}\exp(i\Omega(x,y,z) t+\phi_0)A(x,y,z)dxdydz,\label{eq:fid_dev1}
%\end{align}
%where $\Omega(x,y,z)$ and $A(x,y,z)$ are position dependent. Furthermore, the identity operator $\int\delta(\omega-\Omega)d\omega$ can be inserted into Eq.~\ref{eq:fid_dev1} and change the variable being integrated to frequency instead of positions, and then Eq.~\ref{eq:fid_dev1} become
%\begin{align}
%f(t)&=N\exp(-\frac{t}{\tau})\int_{-\infty}^{+\infty}g(\omega)\exp(i(\omega t + \phi_0))d\omega,\label{eq:fid_non-uniform}\\
%g(\omega)&=\frac{1}{N}\iiint_{-\infty}^{+\infty}\delta(\omega-\Omega(x,y,z))A(x,y,z)dxdydz.
%\label{eq:g_function}
%\end{align}
%where $N$ is a normalization factor so that $\int_{0}^{+\infty}g(\omega)d\omega=1$. Thus, $g(\omega)$ is the NMR frequency spectrum (ignoring the broadening effect due to the exponential decay with time constant $\tau$) for an NMR probe in a non-uniform magnetic field, and it can be interpreted as the signal strength for each frequency component. %According to Eq.~\ref{eq:g_function}, $g(\omega)$ depends not only on the probe properties like the geometry and sensitivity, but also on the shape of the magnetic field. 

%The integral in Eq.~\ref{eq:fid_non-uniform} is a function of $t$, and its general form is 
%\begin{align}
%    E(t)\exp(i\Phi(t))
%    \label{eq:general_complex}
%\end{align}
%as a complex function, and it can be shown that $E(t)$ and $\Phi(t)$ are the amplitude and phase of the Fourier transform of $g(\omega)$. $E(t)$ multiplied by $\exp(-t/\tau)$ determines the envelope of the FID. The broader $g(\omega)$ is, the shorter $E(t)$ is, and therefore large field non-uniformity results in short FIDs. More importantly, the average NMR frequency weighted by $g(\omega)$ equals the time derivative of $\Phi(t)$ at $t=0$:
%\begin{align}
%    \bar{\omega}&=\int_{-\infty}^{+\infty}\omega g(\omega)d\omega\\
%    &=\left. \frac{d\Phi(t)}{dt} \right| _{t=0},
%\end{align}
%and $t=0$ corresponds to the time right before the $\pi/2$-pulse is fired. In the next subsection, the methods of extracting $\Phi(t)$ from an FID signal and determining its time derivative at $t=0$ are described.

%One simple way to construct $\Phi(t)$ from the physical FID function $f_r$ is to determine its zero-crossing times, and after each zero-crossing, $\Phi(t)$ increments by $\pi$. The starting phase is not important because only $d\Phi/dt$ is of concern. This method reduces the number of data points from the number of samples to the number of zero-crossings. Another way to determine $\Phi(t)$ is to use the Hilbert transform. 

The phase function $\Phi(t)$ can be constructed using the Hilbert transform. The Hilbert transform ($\mathcal{H}$) of an arbitrary function $u(t)$ is defined as \cite{Zygmund:1988}:
\begin{align}
    \mathcal{H}\{u(t)\}=\frac{1}{\pi}\lim_{\epsilon \rightarrow 0}\int_{\epsilon}^{+\infty}\frac{u(t+\tau)-u(t-\tau)}{\tau}d\tau.\label{eq:hilbert_transform}
\end{align}
Particularly, the Hilbert transform of $\exp(-t/T_{2})\cos(\omega t)$ ($\omega>0,t>0$) is $\exp(-t/T_{2})\sin(\omega t)$. According to Eq.~\ref{eq:fid_nonuniform}, the physical FID signal $f_{r}(t)$ is essentially a linear superposition of functions $\exp(-t/T_{2})\cos(\omega t+\phi_{0})$ with weight $Ng(\omega)$. Because the Hilbert transform is linear, the Hilbert transform ($f_{i}(t)$) of the FID signal must be the superposition of the $\exp(-t/T_{2})\sin(\omega t+\phi_{0})$ with the same weight. Therefore, 
\begin{align}
    f_{i}(t)&=N\exp(-\frac{t}{T_{2}})\int_{-\infty}^{+\infty}g(\omega)\sin(\omega t + \phi_0)d\omega,\label{eq:fid_imaginary}\\
    &=A(t)\sin(\Phi(t)),\nonumber\\
    &={\text Im}(f(t)).\nonumber
\end{align}
Then the envelope function $A(t)$ and the phase function $\Phi(t)$ of an FID can be obtained by 
\begin{align}
    A(t)&=\sqrt{f_r^2(t)+f_i^2(t)},\label{eq:envelope}\\
    \Phi(t)&=\tan^{-1}(f_i(t)/f_r(t)).\label{eq:phase_hilbert}
\end{align}
The Hilbert transform can be performed via the Fourier transform ($\mathcal{F}$):
\begin{align}
    \mathcal{H}\{f\}=\mathcal{F}^{-1}\{-i\text{sgn}(\omega)\mathcal{F}\{f\}\}, \label{eq:hilbert_transform_fourier}
\end{align}
and therefore Fourier transform algorithms are often used to compute the Hilbert transform of a function.
%First, perform the Fourier transform on the physical FID signal $f_{r}(t)$ obtain its transform $F(\omega)$. Then multiply $+i$ to $F(\omega)$ for $\omega>0$ and $-i$ to $F(\omega)$ for $\omega<0$. Finally, apply the inverse Fourier transform on the modified $F(\omega)$ to get $f_{i}(t)$. 
Because the FID waveforms in this analysis are discrete, in this paper $\mathcal{H}$ and $\mathcal{F}$ represent discrete Hilbert and Fourier transforms.
%Numerically, the discrete Fourier transforms are performed using the Fast Fourier Transform (FFT) algorithm.

The constant initial phase $\phi_0$ in Eq.~\ref{eq:fid_nonuniform} can be factored out, and thus, $\Phi(t)-\phi_0$ can be written explicitly as
\begin{align}
    \Phi(t)-\phi_0=\tan^{-1}\left(\frac{\int_{-\infty}^{+\infty}g(\omega)\sin(\omega t)d\omega}{\int_{-\infty}^{+\infty}g(\omega)\cos(\omega t)d\omega}\right).\label{eq:phase_explicit}
\end{align}
Therefore, $\Phi(t)-\phi_0$ is an odd function of $t$, and its Taylor expansion at $t=0$ contains only odd orders. The third and higher order derivatives of $\Phi(t)$ at $t=0$ are related to higher-order moments of $g(\omega)$ \cite{Cowan_1996}. By fitting the phase function extracted from an FID to a truncated power series
\begin{align}
\Phi_{\text{fit}}(t)=\phi_{0}+p_{1}t+p_{3}t^{3}+p_{5}t^{5}+\cdots,\label{eq:fit_function}
\end{align}
the average frequency $\bar{\omega}$ is then determined, which is the fitted value of $p_{1}$.

To validate this method, FIDs are constructed using artificial $g(\omega)$ functions, and the extracted average frequencies from these FIDs are compared to the truth calculations derived from the $g(\omega)$ functions as shown below. To better simulate the magnetic field in an experiment, the $g(\omega)$ function can be determined using a measured magnetic field map. The response function is calculated using a realistic geometry of the coil and detection material of the magnetometer. In this study, the FID simulation is based on the magnetic field and NMR probes of the Muon $g-2$ experiment \cite{hong2019magnetic}. The magnetic field in the muon beam storage ring is $\sim$1.45~T. The NMR probes for scanning and monitoring the magnetic field have a coil with a length of 1.5~cm and a diameter of 4.6~mm, and the detection material is petroleum jelly filled in a cylindrical cell inside the coil and that extends twice as long as the coil length. The proton-precession frequency in this magnetic field is about 61.79~MHz, and %the high-precision reference signal for the mixing-down 
the local oscillator \cite{SG380} frequency is set to 61.74~MHz so that the frequency of the FID is near 50~kHz. The goal is to have the uncertainty on the measured average magnetic field in the beam-storage volume be below 70~parts-per-billion (ppb), and the budget for uncertainties related to the FID frequency extraction algorithm is 10~ppb. The magnetic field has a peak-to-peak 90~ppm fluctuation around its $\sim$45-m perimeter. The fluctuations are short-ranged, resulting in gradients larger than 1~ppm/mm ($\sim$390~Hz/mm) at many locations. To exemplify the FID frequency extraction, an FID measured in a typical magnetic field with a gradient of 0.3~ppm/mm and a second-order derivative of 5~ppb/mm$^{2}$ along the probe axis is simulated, and the simulated frequency distribution function $g(\omega)$ is shown in Fig.~\ref{fig:LineShape}. Because of the nonzero second-order spatial derivative of the field, $g(\omega)$ is not symmetric and thus $\Phi(t)$ is nonlinear \cite{Cowan_1996}. The FID construction using this $g(\omega)$ function is shown in Fig.~\ref{fig:Fid} together with the extracted envelope function. The extracted phase function is shown in Fig.~\ref{fig:Phase}, where it is fit to Eq.~\ref{eq:fit_function} truncated at the order of $t^{7}$ in the window of 0 to 2.5~ms. The fitted value of $p_{1}$ is different from the true value of $\bar{\omega}$ by 0.1~Hz. The fit performance can be improved by adjusting the fit region and the truncation order of the fit function. For example, if the fit range is shortened to the time when the FID envelope drops to 70\% of its maximum amplitude, and the truncation order is $t^{5}$, the difference between the fitted value and the truth of $\bar{\omega}$ is below 0.01~Hz (0.16~ppb of the magnetic field in the Muon g-2 experiment). In the following studies, this choice of fit range and truncation order is used.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\linewidth]{PublicationGeneratedLineShape.png}
\caption{Frequency distribution function $g(\omega)$ for a simulated FID of an NMR probe that measures a magnetic field with both first-order and second-order derivatives along the probe axial direction. \label{fig:LineShape}}
\end{figure}

\begin{figure}[h!]
\centering
\subfloat[][Fid  and its envelope] {\includegraphics[width=0.49\linewidth]{PublicationFidExampleCombined.png} \label{fig:Fid}}
\subfloat[][Phase]{\includegraphics[width=0.49\linewidth]{PublicationFidPhaseCombined.png}\label{fig:Phase}}
\caption{FID, envelope and phase. The pattern seen in the FID plot is an artifact due to the discretized data points. The insert in Fig.~\ref{fig:Fid} is a magnified view of the FID near $t=0.6$~ms to show its sinusoidal-oscillation pattern. In Fig.~\ref{fig:Phase}, to better visualize the non-linear component of the phase function, $\omega_0 t$ is subtracted from $\Phi(t)$, where $\omega_0$ is an angular frequency close to $\bar{\omega}$. The fit region is magnified.}
\label{fig:env_phi}
\end{figure}

The accuracy of the fit described above is achieved for an FID without noise or artifacts, even with a $\sim$350~Hz full-width-half-maximum (FWHM) of the corresponding $g(\omega)$. As long as the fit range is within the Taylor series convergence radius of $\Phi(t)$, the fit accuracy can be improved by increasing the truncation order. However, the fit accuracy is also limited by the effects of artifacts, which will be described in Sec.~\ref{sec:artifact_uncertainty}.


==> MethodTim.tex <==
\section{FID Frequency Extraction Methods}
\label{sec:method}

%Note: omega IS frequency, so I don't think "angular" is needed just to emphasize the 2pi

%I think the first sentence would be better characterized as the contribution to the FID for a volume of sample $dV$. This is because you call the FID signal, the signal in the coil, which is a superposition, even if there is a uniform field and single frequency - i.e. it depends (as you know) on the coil size, etc. So an alternative 1st sentence is
%The FID is a superposition of the voltages induced in the coil from precessing magnetization throughout the sample. The contribution to the FID from a volume element $dV$ at a specific position is
%\begin{align}
%f(t)=A\exp(-t/T_{2})\exp\left(i(\omega t+\phi_0)\right)\label{eq:fid_uniform}, 
%\end{align}
%where the down-mixed frequency is $\omega=\gamma B(\vec r)-\gamma_r$, and $A$\vec r$$ is the initial contribution to the signal amplitude. 

%You use f(t) to indicate more than one thing. Try $\tilde f$, $\bar f$ or even $F(t)$ or something

%So actually, I think it would be best to just start with the full FID: 
%
% At the end you have "truth" i.e $\bar\gamma$ - so is this an explicit integral?
%
%What is "fit performance"?
%
%Note absolute values: $|\bar{\omega}-p_{1}|<0.01$
%
%What is "Taylor series convergence radius" 
% 
%At the end you use 7th order and 2.5 ms but then seem to settle on 5th order and end time of 70% of initial FID amplitude. I think you want to show the dependence on order and time/SNR. I would reverse these - what you end up using and then a variant.

{\color{blue}

The FID is a superposition of the voltages induced in the coil from precessing magnetization throughout the sample which vary in frequency due to a non-uniform magnetic field and vary in amplitude due to position with respect to the NMR coil. This can be modeled
\begin{align}
f(t)&=N\exp(-\frac{t}{T_{2}})\int_{-\infty}^{+\infty}g(\omega)\exp(i(\omega t + \phi_0))d\omega,\label{eq:fid_nonuniform}
\end{align}
where $N$ is a normalization constant, $T_2$ is the intrinsic transverse decay time of the sample, and $g(\omega)d\omega$ is the signal generated within an angular frequency range $(\omega,\omega+d\omega)$ due to the superposition of contributions from all parts of the sample. 
%In a uniform magnetic field, the FID signal $f(t)$ can be modeled as
%\begin{align}
%f(t)=A\exp(-t/T_{2})\exp\left(i(\omega t+\phi_0)\right)\label{eq:fid_uniform}, 
%\end{align}
%where $\omega$ is the nuclear spin precession angular frequency after the down-mixing, and $A$ is its initial signal amplitude. The decay time constant $T_{2}$ describes the intrinsic relaxation of the transverse component of the nuclear spin polarization \cite{Slichter:1990}, and it depends on the sample material. %If the FID signal is mixed-down before digitization, $\omega$ is the NMR frequency after the down mixing. 
%The oscillation factor $\exp(i(\omega t+\phi_0))$ of the FID is expressed in the complex form to simplify later derivations, and the physical signal $f_r$ is the real part of this complex function. 
The function $f(t)$ is complex, and the measured signal is its real part $f_r(t)$. 
%If the magnetic field is not uniform the signal in the NMR coil is a superposition of FIDs with different frequencies and amplitudes. Suppose the signal generated within an angular frequency range $(\omega,\omega+d\omega)$ has an amplitude of $g(\omega)d\omega$, the net signal is given by the superposition
%\begin{align}
%f(t)&=N\exp(-\frac{t}{T_{2}})\int_{-\infty}^{+\infty}g(\omega)\exp(i(\omega t + \phi_0))d\omega,\label{eq:fid_nonuniform}
%\end{align}. 
The FID function can be expressed in the form of a general complex function
\begin{align}
    f(t)=A(t)\exp(i\Phi(t)),
    \label{eq:general_complex}
\end{align}
where $A(t)$ and $\Phi(t)$ are real. We want to determine the frequency corresponding to the a volume average of the magnetic field weighted by the signal contribution from positions within the sample. 
According to Ref.~\cite{Cowan_1996}, the average NMR frequency $\bar{\omega}$ weighted by $g(\omega)$ can be determined by calculating the derivative of $\Phi(t)$ at $t=0$:
\begin{align}
    \bar{\omega}&=\int_{-\infty}^{+\infty}\omega g(\omega)d\omega\\
    &=\left. \frac{d\Phi(t)}{dt} \right| _{t=0},
\end{align}
and $t=0$ corresponds to the time when the $\pi/2$-pulse starts. %This average frequency corresponds to the average field sensed by the probe weighted by the signal amplitude for the frequency interval. 

%Assume the magnetic field being measured is in the $hat{y}$-direction, and the axial of the NMR probe coil is along the $\hat{z}$-direction. The $\pi/2$-pulse flips the magnetic polarization due to the proton magnetic moment from the $\hat{y}$ direction into the $x-z$ plane. After the $\pi/2$-pulse, the FID signal generated by the precession of the nuclear magnetic polarization can be modeled as 
%\begin{align}
%f(t)&=A\exp(-\frac{t}{\tau})\exp(i(\Omega t + \phi_0)),\label{eq:fid_uniform}\\
%\frac{1}{\tau}&=\frac{1}{T_1}+\frac{1}{T_2},\nonumber
%\end{align}
%where $\Omega$ is the NMR frequency, and $\phi_0$ is a constant initial phase. If the FID is mixed with a standard-frequency signal, then $\Omega=\omega_{s}-\omega_{R}$. The time constants $T_1$ and $T_2$ depend on the detection material, but not the nonuniformity of the magnetic field. Eq.~\ref{eq:fid_uniform} uses the complex form to simplify the calculation, and the physical signal is the real part of it. 

%In a non-uniform field, protons at different positions precess at different angular frequencies. The amplitude contributions from different positions are also different, because the $\pi/2$-pulse strength, sensitivity of the coil, and potentially the detection material distribution are not uniform. For a macroscopically small volume $dV=dxdydz$ in which the magnetic field non-uniformity is negligible, the signal generated in this volume can still be modeled by Eq.~\ref{eq:fid_uniform}. At the macroscopic distance the magnetic field generated by the precessing nuclear magnetic polarization is rather small comparing to the main magnetic field, so the signals generated by different volumes are independent and the total signal is the superposition of them:
%\begin{align}
%    f(t)&=\exp(-\frac{t}{\tau})\iiint_{-\infty}^{+\infty}\exp(i\Omega(x,y,z) t+\phi_0)A(x,y,z)dxdydz,\label{eq:fid_dev1}
%\end{align}
%where $\Omega(x,y,z)$ and $A(x,y,z)$ are position dependent. Furthermore, the identity operator $\int\delta(\omega-\Omega)d\omega$ can be inserted into Eq.~\ref{eq:fid_dev1} and change the variable being integrated to frequency instead of positions, and then Eq.~\ref{eq:fid_dev1} become
%\begin{align}
%f(t)&=N\exp(-\frac{t}{\tau})\int_{-\infty}^{+\infty}g(\omega)\exp(i(\omega t + \phi_0))d\omega,\label{eq:fid_non-uniform}\\
%g(\omega)&=\frac{1}{N}\iiint_{-\infty}^{+\infty}\delta(\omega-\Omega(x,y,z))A(x,y,z)dxdydz.
%\label{eq:g_function}
%\end{align}
%where $N$ is a normalization factor so that $\int_{0}^{+\infty}g(\omega)d\omega=1$. Thus, $g(\omega)$ is the NMR frequency spectrum (ignoring the broadening effect due to the exponential decay with time constant $\tau$) for an NMR probe in a non-uniform magnetic field, and it can be interpreted as the signal strength for each frequency component. %According to Eq.~\ref{eq:g_function}, $g(\omega)$ depends not only on the probe properties like the geometry and sensitivity, but also on the shape of the magnetic field. 

%The integral in Eq.~\ref{eq:fid_non-uniform} is a function of $t$, and its general form is 
%\begin{align}
%    E(t)\exp(i\Phi(t))
%    \label{eq:general_complex}
%\end{align}
%as a complex function, and it can be shown that $E(t)$ and $\Phi(t)$ are the amplitude and phase of the Fourier transform of $g(\omega)$. $E(t)$ multiplied by $\exp(-t/\tau)$ determines the envelope of the FID. The broader $g(\omega)$ is, the shorter $E(t)$ is, and therefore large field non-uniformity results in short FIDs. More importantly, the average NMR frequency weighted by $g(\omega)$ equals the time derivative of $\Phi(t)$ at $t=0$:
%\begin{align}
%    \bar{\omega}&=\int_{-\infty}^{+\infty}\omega g(\omega)d\omega\\
%    &=\left. \frac{d\Phi(t)}{dt} \right| _{t=0},
%\end{align}
%and $t=0$ corresponds to the time right before the $\pi/2$-pulse is fired. In the next subsection, the methods of extracting $\Phi(t)$ from an FID signal and determining its time derivative at $t=0$ are described.

%One simple way to construct $\Phi(t)$ from the physical FID function $f_r$ is to determine its zero-crossing times, and after each zero-crossing, $\Phi(t)$ increments by $\pi$. The starting phase is not important because only $d\Phi/dt$ is of concern. This method reduces the number of data points from the number of samples to the number of zero-crossings. Another way to determine $\Phi(t)$ is to use the Hilbert transform. 

The phase function $\Phi(t)$ can be constructed using the Hilbert transform. The Hilbert transform ($\mathcal{H}$) of an arbitrary function $u(t)$ is defined as \cite{Zygmund:1988}:
\begin{align}
    \mathcal{H}\{u(t)\}=\frac{1}{\pi}\lim_{\epsilon \rightarrow 0}\int_{\epsilon}^{+\infty}\frac{u(t+\tau)-u(t-\tau)}{\tau}d\tau.\label{eq:hilbert_transform}
\end{align}
Particularly, the Hilbert transform of $\exp(-t/T_{2})\cos(\omega t)$ ($\omega>0,t>0$) is $\exp(-t/T_{2})\sin(\omega t)$. According to Eq.~\ref{eq:fid_nonuniform}, the physical FID signal $f_{r}(t)$ is essentially a linear superposition of  $\exp(-t/T_{2})\cos(\omega t+\phi_{0})$ with weight $Ng(\omega)$. Because the Hilbert transform is linear, the Hilbert transform ($f_{i}(t)$) of the FID signal must be the superposition of the $\exp(-t/T_{2})\sin(\omega t+\phi_{0})$ with the same weight. Therefore, 
\begin{align}
    f_{i}(t)&=N\exp(-\frac{t}{T_{2}})\int_{-\infty}^{+\infty}g(\omega)\sin(\omega t + \phi_0)d\omega,\label{eq:fid_imaginary}\\
    &=A(t)\sin(\Phi(t)),\nonumber\\
    &={\text Im}(f(t)).\nonumber
\end{align}
Then the envelope function $A(t)$ and the phase function $\Phi(t)$ of an FID can be obtained by 
\begin{align}
    A(t)&=\sqrt{f_r^2(t)+f_i^2(t)},\label{eq:envelope}\\
    \Phi(t)&=\tan^{-1}(f_i(t)/f_r(t)).\label{eq:phase_hilbert}
\end{align}
The Hilbert transform can be is related to the Fourier transform ($\mathcal{F}$) by:
\begin{align}
    \mathcal{H}\{f\}=\mathcal{F}^{-1}\{-i\text{sgn}(\omega)\mathcal{F}\{f\}\}, \label{eq:hilbert_transform_fourier},
\end{align}
and therefore Fourier transform algorithms are often used to compute the Hilbert transform of a function.
%First, perform the Fourier transform on the physical FID signal $f_{r}(t)$ obtain its transform $F(\omega)$. Then multiply $+i$ to $F(\omega)$ for $\omega>0$ and $-i$ to $F(\omega)$ for $\omega<0$. Finally, apply the inverse Fourier transform on the modified $F(\omega)$ to get $f_{i}(t)$. 
Because the FID waveforms in this analysis are discrete, in this paper $\mathcal{H}$ and $\mathcal{F}$ represent discrete Hilbert and Fourier transforms.
%Numerically, the discrete Fourier transforms are performed using the Fast Fourier Transform (FFT) algorithm.

The constant initial phase $\phi_0$ in Eq.~\ref{eq:fid_nonuniform} can be factored out, and thus, $\Phi(t)-\phi_0$ can be written explicitly as
\begin{align}
    \Phi(t)-\phi_0=\tan^{-1}\left(\frac{\int_{-\infty}^{+\infty}g(\omega)\sin(\omega t)d\omega}{\int_{-\infty}^{+\infty}g(\omega)\cos(\omega t)d\omega}\right).\label{eq:phase_explicit}
\end{align}
Therefore, $\Phi(t)-\phi_0$ is an odd function of $t$, and its Taylor expansion at $t=0$ contains only odd orders. The third and higher order derivatives of $\Phi(t)$ at $t=0$ are related to higher-order moments of $g(\omega)$ \cite{Cowan_1996}. The phase function is fit to a truncated power series
\begin{align}
\Phi_{\text{fit}}(t)=\phi_{0}+p_{1}t+p_{3}t^{3}+p_{5}t^{5}+\cdots,\label{eq:fit_function},
\end{align}
and $\bar{\omega}=p_{1}$.

The validity of the method was studied with simulated FIDs are constructed with artificial $g(\omega)$ functions based on magnetic field maps measured in the $g-2$ experiment \cite{hong2019magnetic} and realistic sample/coil geometry.  %(is probe actually defined anywhere?).
% The extracted average frequencies $\bar{\omega}$ are compared to analytic results derived from the $g(\omega)$ functions as shown below. 
%To better simulate the magnetic field in an experiment, the $g(\omega)$ function can be determined using a measured magnetic field map. 
%The response function is calculated using a realistic geometry of the coil and detection material of the probe. 
%In this study, the FID simulation is based on the magnetic field and NMR probes of the Muon $g-2$ experiment \cite{hong2019magnetic}. 
%The magnetic field in the muon beam storage ring is $\sim$1.45~T.
 The NMR probes %(is probe actually defined anywhere?).
 for scanning and monitoring the magnetic field have a coil with a length of 1.5~cm and a diameter of 4.6~mm, and the sample is an approximately 3~cm long, 4 mm diameter cylinder of  petroleum jelly. The proton-precession frequency at the nominal 1.45 T magnetic field is about 61.79~MHz, and %the high-precision reference signal for the mixing-down 
the reference frequency  \cite{SG380} is set to $\gamma_r=$ 61.74~MHz so that the frequency of the FID is near 50~kHz.
%This should go in the introduction!
% To achieve the goal of 70 ppb on the uncertainty of the measured average magnetic field in the beam-storage volume (is beam storage volume or beam or storage volume defined?) the uncertainty related to the FID frequency extraction algorithm should be less than 10~ppb. 
 The magnetic field has azimuthal gradients as large as ($1~|mu$~T/mm) at several locations. 
 %a peak-to-peak 90~ppm fluctuations around its $\sim$45-m perimeter. The fluctuations are short-ranged, resulting in gradients larger than 1~ppm/mm ($\sim$390~Hz/mm) at many locations. 
 A gradient of 0.3~ppm/mm and a second-order derivative of 5~ppb/mm$^{2}$ along the sample axis produced $g(\omega)$ is shown in Fig.~\ref{fig:LineShape}. Due to the second-order spatial derivative of the field, $g(\omega)$ is not symmetric and thus $\Phi(t)$ is nonlinear \cite{Cowan_1996}. The FID construction using this $g(\omega)$ function is shown in Fig.~\ref{fig:Fid} together with the extracted envelope function. The extracted phase function is shown in Fig.~\ref{fig:Phase}, along with a fit to Eq.~\ref{eq:fit_function} truncated at order of $t^{7}$  over the range 0 to 2.5~ms. 
 The difference of the fit  and average frequency determined from (integrating the field over the sample) is  $|\bar{\omega}-p_{1}|=0.1$~Hz. The fit accuracy(?) can be improved by adjusting the fit region and the truncation order of the fit function. For example, if the end of the fit range is reduced to the time when the FID envelope drops to 70\% of its maximum amplitude, and the truncation order is $t^{5}$, the difference between the fitted value and the truth of $|\bar{\omega}-p_{1}|<0.01$~Hz, corresponding to 0.16~ppb  for the magnetic field in the Muon g-2 experiment. 
 %In the following studies, this choice of fit range and truncation order is used.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\linewidth]{PublicationGeneratedLineShape.png}
\caption{Frequency distribution function $g(\omega)$ for a simulated FID of an NMR probe that measures a magnetic field with both first-order and second-order derivatives along the probe axial direction. \label{fig:LineShape}}
\end{figure}

\begin{figure}[h!]
\centering
\subfloat[][Fid  and its envelope] {\includegraphics[width=0.49\linewidth]{PublicationFidExampleCombined.png} \label{fig:Fid}}
\subfloat[][Phase]{\includegraphics[width=0.49\linewidth]{PublicationFidPhaseCombined.png}\label{fig:Phase}}
\caption{FID, envelope and phase. The pattern seen in the FID plot is an artifact due to the discretized data points. The insert in Fig.~\ref{fig:Fid} is a magnified view of the FID near $t=0.6$~ms to show its sinusoidal-oscillation pattern. In Fig.~\ref{fig:Phase}, to better visualize the non-linear component of the phase function, $\omega_0 t$ is subtracted from $\Phi(t)$, where $\omega_0$ is an angular frequency close to $\bar{\omega}$. The fit region is magnified.}
\label{fig:env_phi}
\end{figure}

The accuracy of the fit described above is achieved for an FID without noise or artifacts, with a $\sim$350~Hz full-width-half-maximum (FWHM) of the corresponding $g(\omega)$. As long as the fit range is within the Taylor series convergence radius of $\Phi(t)$, the fit accuracy can be improved by increasing the truncation order. However, the fit accuracy is also limited by the effects of artifacts, which will be described in Sec.~\ref{sec:artifact_uncertainty}.

}

